GraphPI: Efficient Protein Inference with Graph Neural Networks

The integration of deep learning approaches in biomedical research has been transformative, enabling breakthroughs in various applications. Despite these strides, its application in protein inference is impeded by the scarcity of extensively labeled datasets, a challenge compounded by the high costs and complexities of accurate protein annotation. In this study, we introduce GraphPI, a novel framework that treats protein inference as a node classification problem. We treat proteins as interconnected nodes within a protein-peptide-PSM graph, utilizing a Graph Neural Network-based architecture to elucidate their interrelations. To address label scarcity, we train the model on a set of unlabeled public protein datasets with pseudo-labels derived from an existing protein inference algorithm, enhanced by self-training to iteratively refine labels based on confidence scores. Contrary to prevalent methodologies necessitating dataset-specific training, our research illustrates that GraphPI, due to the well normalized nature of Percolator features, exhibits universal applicability without dataset-specific fine-tuning, a feature that not only mitigates the risk of overfitting but also enhances computational efficiency. Our empirical experiments reveal notable performance on various test datasets and deliver significantly reduced computation times compared to common protein inference algorithms.

==> chapters/Experiments.tex <==
\section{Results and Discussion}

\subsection{Comparison Study}


The performances of all methods are evaluated by the receiver operator characteristic (ROC) curve, which plots the number of true positive proteins (i.e. the number of ground truth proteins) as a function of entrapment FDR (the portion of entrapment proteins in the identified list). The curve is plotted by varying the FDR threshold above which a protein will appear in the identified list. Given that the test datasets all have ground truth attached to them, we can evaluate based on empirical FDR instead of decoy FDR. Since we are mostly interested in the performance of the methods when the FDR is small, we plot the curve within the entrapment FDR range of $[0.01, 0.05]$. The results are shown in Figure~\ref{fig: comparison1}.

\begin{figure}[t!]
%\captionsetup[subfigure]%{justification=Centering}
\centering
\begin{subfigure}[t]{0.49\textwidth}
\centering
    \includegraphics[width=3.2in]{figures/iPRG2016_A_plotting_roc.eps}
    \caption{iPRG2016 A}
    \label{fig: iprg_a_roc}
\end{subfigure}\hspace{\fill} % maximize horizontal separation
\hfill
\begin{subfigure}[t]{0.49\textwidth}
\centering
    \includegraphics[width=3.2in]{figures/iPRG2016_B_plotting_roc.eps}
    \caption{iPRG2016 B}
    \label{fig: iprg_b_roc}
\end{subfigure}

 % Add a line break after the second image

\begin{subfigure}[t]{0.49\textwidth}
\centering
    \includegraphics[width=3.2in]{figures/iPRG2016_AB_plotting_roc.eps}
    \caption{iPRG2016 AB}
    \label{fig: iprg_ab_roc}
\end{subfigure}\hspace{\fill} % maximize horizontal separation
\hfill
\begin{subfigure}[t]{0.49\textwidth}
\centering
    \includegraphics[width=3.2in]{figures/yeast_plotting_roc.eps}
    \caption{Yeast}
    \label{fig: yeast_roc}
\end{subfigure}

%\newline % Add a line break after the fourth image

\begin{subfigure}[t]{0.49\textwidth}
\centering
    \includegraphics[width=3.2in]{figures/ups2_plotting_roc.eps}
    \caption{UPS2}
    \label{fig: ups2_roc}
\end{subfigure}\hspace{\fill} % maximize horizontal separation
\hfill
\begin{subfigure}[t]{0.49\textwidth}
\centering
    \includegraphics[width=3.2in]{figures/18mix_plotting_roc.eps}
    \caption{18Mix}
    \label{fig: 18mix_roc}
\end{subfigure}

\caption{ROC curve (entrapment FDR vs. number of true proteins) of various models on the benchmark datasets. We encountered an error while running DeepPep on 18Mix, thus it is excluded.}
\label{fig: comparison1}
\end{figure}


Overall, our method shows competing performance across all datasets. For both the iPRG2016 A and B datasets, GraphPI is the only one that can compete with Epifany in terms of identification performance. In addition, our ROC curves rise faster than any other method in these two datasets, showing improved performance in the low FDR range. In iPRG2016 AB, GraphPI ranks the second throughout the whole FDR range, only falling behind PIA, which performs extraordinarily well in this dataset. In the Yeast dataset, our method again shows overall best performance. In the UPS2 dataset, GraphPI acquires identification performance similar to that of Epifany, surpassing Fido, PIA, and DeepPep.  Additionally, we rank the top along with Epifany for the 18Mix dataset. It is worth noting that, while Epifany can produce state-of-the-art performance in iPRG2016 A and B, it falls short in other datasets like AB and Yeast, but our approach retains competitive and consistent performance across all datasets. 

We also compared the pAUC based on FDR from $1\%$ to $5\%$ of test methods, summarized in Figure~\ref{fig: comparison2}. The results are consistent with our previous analysis, with our method achieving the top performance in iPRG2016 A, B, Yeast and 18Mix, being second in iPRG2016 AB and UPS2.


\begin{figure}[t!]
%\captionsetup[subfigure]%{justification=Centering}
\centering
\begin{subfigure}[t]{0.49\textwidth}
\centering
    \includegraphics[width=3.2in]{figures/iPRG2016_A_plotting_pauc.eps}
    \caption{iPRG2016 A}
    \label{fig: iprg_a_pauc}
\end{subfigure}\hspace{\fill} % maximize horizontal separation
\hfill
\begin{subfigure}[t]{0.49\textwidth}
\centering
    \includegraphics[width=3.2in]{figures/iPRG2016_B_plotting_pauc.eps}
    \caption{iPRG2016 B}
    \label{fig: iprg_b_pauc}
\end{subfigure}

 % Add a line break after the second image

\begin{subfigure}[t]{0.49\textwidth}
\centering
    \includegraphics[width=3.2in]{figures/iPRG2016_AB_plotting_pauc.eps}
    \caption{iPRG2016 AB}
    \label{fig: iprg_ab_pauc}
\end{subfigure}\hspace{\fill} % maximize horizontal separation
\hfill
\begin{subfigure}[t]{0.49\textwidth}
\centering
    \includegraphics[width=3.2in]{figures/yeast_plotting_pauc.eps}
    \caption{Yeast}
    \label{fig: yeast_pauc}
\end{subfigure}

%\newline % Add a line break after the fourth image

\begin{subfigure}[t]{0.49\textwidth}
\centering
    \includegraphics[width=3.2in]{figures/ups2_plotting_pauc.eps}
    \caption{UPS2}
    \label{fig: ups2_pauc}
\end{subfigure}\hspace{\fill} % maximize horizontal separation
\hfill
\begin{subfigure}[t]{0.49\textwidth}
\centering
    \includegraphics[width=3.2in]{figures/18mix_plotting_pauc.eps}
    \caption{18Mix}
    \label{fig: 18mix_pauc}
\end{subfigure}

\caption{pAUC (partial AUC) score of various models on the benchmark datasets.}
\label{fig: comparison2}

\end{figure}



\subsection{Computational Efficiency}
To demonstrate the computational efficiency of GraphPI, we report the runtimes in minutes on the Yeast dataset, which is the largest dataset in our test data. The runtimes are measured on an Intel Core i7 8700K processor. Every algorithm is executed with 12 threads to take advantage of parallelism. GPU acceleration is disabled during inference time to make the comparison fair.

Our method shows a significant advantage when compared to other models, especially Bayesian methods, like Fido or Epifany. On the Yeast dataset, our method takes only 88 seconds to run, while Epifany takes over 14 minutes. Partially this is due to the inherent speed advantage of neural networks over Bayesian networks. On the other hand, Epifany and Fido need to run a grid search of their parameters $\alpha$, $\beta$, and $\gamma$ for every test dataset, while our approach does not need such a procedure, further improving efficiency.



Additionally, the design of the GNN model architecture guarantees that the runtime scales linearly with respect to the dataset size (number of proteins to be evaluated), eliminating the undesired effect of higher-order scaling. Figure~\ref{fig: yeast_time} shows the runtime of our method plotted against the number of proteins in the dataset, demonstrating the linear scaling.

The efficiency of our method enables its application in large-scale datasets, which might be impossible for other methods due to computational constraints. 

\begin{figure}[t!]
%\captionsetup[subfigure]%{justification=Centering}
\centering
\begin{subfigure}[t]{0.49\textwidth}
\centering
    \includegraphics[width=3.2in]{figures/yeast_time.eps}
    \caption{}
    \label{fig: yeast_time}
\end{subfigure}%\hspace{\fill} % maximize horizontal separation
\hfill
\begin{subfigure}[t]{0.49\textwidth}
\centering
    \includegraphics[width=3.2in]{figures/linear_time.eps}
    \caption{}
    \label{fig: linear_time}
\end{subfigure}
\caption{(a) Inference time of the benchmarked methods on the Yeast dataset. (b) Scaling of inference time for our model on datasets of different sizes.}
\end{figure}


\subsection{Extended Investigation}
\subsubsection{Experiments on Target-Decoy Labels}
Noticing that Barista~\citep{spivak2012direct} is removed from the latest version of Crux~\citep{mcilwain2014crux}, we create a comparable model using our GNN network as the foundational architecture. We trained this model on each test dataset, designating decoy proteins as negative samples and the remainder as positive. Adhering to Barista's documented procedures, we employed 5-fold cross-validation, averaging protein scores across the five models. We've termed this model ``Ours with Target Decoy Training''.

\begin{figure}[t!]
%\captionsetup[subfigure]%{justification=Centering}
\centering
\begin{subfigure}[t]{0.49\textwidth}
\centering
    \includegraphics[height=5.3cm]{figures/iPRG2016_A_plotting_roc_td.eps}
    \caption{iPRG2016 A}
    \label{fig: iprg_a_roc}
\end{subfigure}\hspace{\fill} % maximize horizontal separation
\hfill
\begin{subfigure}[t]{0.49\textwidth}
\centering
    \includegraphics[width=3.2in]{figures/iPRG2016_B_plotting_roc_td.eps}
    \caption{iPRG2016 B}
    \label{fig: iprg_b_roc}
\end{subfigure}

 % Add a line break after the second image

\begin{subfigure}[t]{0.49\textwidth}
\centering
    \includegraphics[width=3.2in]{figures/iPRG2016_AB_plotting_roc_td.eps}
    \caption{iPRG2016 AB}
    \label{fig: iprg_ab_roc}
\end{subfigure}\hspace{\fill} % maximize horizontal separation
\hfill
\begin{subfigure}[t]{0.49\textwidth}
\centering
    \includegraphics[width=3.2in]{figures/yeast_plotting_roc_td.eps}
    \caption{Yeast}
    \label{fig: yeast_roc}
\end{subfigure}

%\newline % Add a line break after the fourth image

\begin{subfigure}[t]{0.49\textwidth}
\centering
    \includegraphics[width=3.2in]{figures/ups2_plotting_roc_td.eps}
    \caption{UPS2}
    \label{fig: ups2_roc}
\end{subfigure}\hspace{\fill} % maximize horizontal separation
\hfill
\begin{subfigure}[t]{0.49\textwidth}
\centering
    \includegraphics[width=3.2in]{figures/18mix_plotting_roc_td.eps}
    \caption{18Mix}
    \label{fig: 18mix_roc}
\end{subfigure}

\caption{ROC curve (entrapment FDR vs. number of true proteins) of GraphPI and GraphPI with Target-Decoy Training on the benchmark datasets.}
\label{fig: comparison_td}
\end{figure}
The ROC curves of our GraphPI and the target-decoy setting is plotted in Figure \ref{fig: comparison_td}. It is evident that while this training setting yields favorable outcomes in the iPRG 2016 AB and UPS2 datasets, it falls short in datasets featuring shared peptides among proteins. This limitation stems from the fact that decoy proteins typically do not share peptides with target proteins, leading to a training gap where the model lacks exposure to examples necessitating differentiation between proteins that share peptides. Our approach effectively addresses this issue by incorporating pseudo-labels from Epifany which additionally imposes penalization on degenerate proteins.

\subsubsection{Analysis on Epifany Results}
\label{sec: case study}
The benefit of GraphPI, a data-driven deep-learning-based approach, is its ability to learn the contribution of each peptide to its parental protein through the data distribution of a common set of datasets. In contrast, Epifany relies on prior probabilities and makes strong assumptions about the data distribution, which can lead to inaccurate protein scores. We provide two visual examples in the following paragraphs, supported by explanations that demonstrate the limitations of Epifany in dealing with certain types of proteins.

\paragraph{Protein prior distribution presents an important role:}
In situations where a peptide has multiple siblings, Epifany tends to downweight the contribution of the peptide score and place greater reliance on the prior score of the protein, particularly in cases where there is no other supporting evidence (i.e., non-degenerate peptides connecting to the protein). This can lead to inaccuracies in protein inference, especially when the prior score of the protein is high and the dataset contains many peptides with shared proteins. We demonstrate an example of this phenomenon in Figure~\ref{fig: case study - protein prior a}, where the highlighted protein is a decoy protein that should not have received a high score, yet Epifany assigns a score that is close to its protein prior score, which is around 0.7. This is attributed to the fact that the prior score of proteins is optimized by the grid search program of Epifany based on Decoy FDR, which has the risk of overfitting the distribution of decoy rather than the actually contaminated proteins.

\begin{figure}[t!]
%\captionsetup[subfigure]%{justification=Centering}

\centering
\begin{subfigure}[t]{1\textwidth}
\centering
    \includegraphics[height=0.8cm]{k_figures/legend_for_case_study.eps}
\end{subfigure}
\newline
\centering
\begin{subfigure}[t]{0.43\textwidth}
\centering
    \includegraphics[height=5cm]{k_figures/case_study_protein_prior_b.eps}
    \caption{}
    \label{fig: case study - protein prior a}
\end{subfigure}%\hspace{\fill} % maximize horizontal separation
%\hfill
% \begin{subfigure}[t]{0.28\textwidth}
% \centering
%     \includegraphics[height=4cm]{figures/case_study_protein_prior_a.eps}
%     \caption{}
%     \label{fig: case study - protein prior b}
% \end{subfigure}
\begin{subfigure}[t]{0.54\textwidth}
\centering
    \includegraphics[height=5cm]{k_figures/case_study_protein_degenerate_a.eps}
    \caption{}
    \label{fig: case study - protein degenerate a}
\end{subfigure}
\caption{\textcolor{red}{In (a)\&(b), the orange circle represents a peptide with its peptide identification score inside, while the blue circle represents a protein. The scores generated by both Epifany and our model are given for the highlighted protein in each graph, respectively. Specifically, (a) shows the bipartite graphs for the selected proteins and their connected peptides from dataset ``PXD005388''. The protein prior is set to 0.7 based on the grid search program of Epifany. The highlighted protein is a decoy protein, which should has a lower score. (b) shows the bipartite graph for proteins selected from the dataset ``iPRG2016 AB''. The highlighted protein is a true protein, which should have a higher score.}}
\end{figure}

\paragraph{Epifany has strong penalization on degenerate proteins:} We use Figure~\ref{fig: case study - protein degenerate a} as an example for illustration: Specifically, the highlighted protein present in the figure is supposed to belong to the true protein group (having higher protein scores). However, Epifany assigns a relatively lower score to it regardless of the high-score peptides that connect to it. The reason behind this is that Epifany assigns a strong prior to peptides that have connections to multiple proteins, having the purpose of lowering their contribution to each parental protein. Specifically, Epifany sets the probability of a peptide that a certain number of proteins can generate to $1/N$, where $N$ is the number of proteins that the peptide is connected to. This prior probability affects the posterior probability score of the peptide, leading to a significant penalty in the contribution of the peptide to the calculation of each parental protein score. This approach gives Epifany superior performance in iPRG2016 A and B where most true proteins do not have degenerated peptides connected, but the performance on other datasets are lacking. 

\subsubsection{Learning beyond Epifany Scores}

Some may posit that GraphPI, which is trained on Epifany's pseudo-labels, might merely mimic Epifany's outputs without surpassing its performance. We argue that the divergence between GraphPI and Epifany can be distilled into three primary distinctions. 
\paragraph{Generalization over overfitting:}
As elucidated earlier in the case study, Epifany is prone to overfitting, particularly given its optimization strategy on priors anchored in Decoy FDR. In contrast, the training of GraphPI harnesses a set of public protein datasets. By building upon Epifany's results generated from diverse datasets, GraphPI inherently promotes broader generalization capabilities. As shown in both Figure~\ref{fig: case study - protein prior a} and Figure~\ref{fig: case study - protein degenerate a}, our method is able to produce a relatively lower score for the decoy protein and a higher score for the true protein, whereas the scores generated from Epifany is either inflated or deflated primarily due to its overfitting of prior probabilities on decoys of individual datasets.

\paragraph{Discerning label incorporation:}
In our label-generation mechanisms, decoy proteins, known to be artificial constructs and absent from biological samples, are consistently tagged as negative, irrespective of the scoring of Epifany. This information enables GraphPI to learn patterns surpassing those identified solely by Epifany. 
Supporting this claim, a comparison of GraphPI's performance with and without the presence of decoy proteins is shown in Table~\ref{table:decoy_ablation_1}. It is evident that the absence of decoy proteins significantly hampers our model's performance.

\begin{table}[H]
    \centering
    \begin{tabular}{| l|l| }
    \hline
    \textbf{Setting} & \textbf{True Positives} \\
    \hline
    Normal Train Data & 187 \\
    \hline
    Without Decoy & 176 \\
    \hline
    Decoys within 5\% FDR as Positive Samples & 183 \\
    \hline
    \end{tabular}
    \caption{Number of true positive (TP) proteins identified by our algorithm, with decoy proteins, without decoy proteins, or with decoys within 5\% FDR labeled as positive proteins. The numbers are acquired under 5\% entrapment FDR, from iPRG2016 B dataset, with only pseudo-labeled training (without self-training) to demonstrate the performance difference.}
    \label{table:decoy_ablation_1}
\end{table}

Nonetheless, an argument could be made that incorporating decoy proteins merely expands the training set, which in turn leads to enhanced performance. To address this concern, we conducted another experiment, where decoy proteins within a 5\% FDR threshold are labeled as positive (mimicking their incorrect identification by Epifany), and the remaining decoy proteins are labeled as negative. In this scenario, positive and negative sample labels are derived by thresholding Epifany's scores based on a 5\% FDR, resulting in labels that precisely match those obtained from Epifany. The results in Table~\ref{table:decoy_ablation_1} show that while integrating decoy data as hard negatives does enhance the model's efficacy, the presence of a few decoy proteins in the positive class can impair performance relative to our standard configuration.

\paragraph{Tailored GNN Architecture, Graph Design, and Self-Training} Another aspect of GraphPI's enhanced capability is its GNN architecture, specifically tailored for a tripartite graph encompassing proteins, peptides, and PSMs.  This tailored structure adeptly captures the complex relationships within proteomic data, reducing the likelihood of overfitting to inaccuracies in Epifany's initial labels. Complementing this, GraphPI employs iterative self-training to refine these pseudo-labels from Epifany. This process allows our model to continually learn and adjust, potentially rectifying inaccuracies in the initial labels.

\subsubsection{Accuracy of FDR Estimation}

We provided an additional analysis on the relationship between entrapment FDR and decoy FDR in the Supporting Material. Generally speaking, our method provides less conservative FDR estimates than Epifany, while being more conservative than other methods in our comparison.



==> chapters/Introduction.tex <==
\section{Introduction}

Protein inference refers to the process of determining the proteins present in a biological sample by analyzing the peptides detected through MS/MS experiments. It is an important area of research in proteomics because accurate identification of proteins is critical for understanding their functions and roles in biological systems. Protein inference results serve as the foundation for various downstream applications, including the identification of biomarkers, drug targets, and the annotation of protein functions. During a MS/MS experiment, proteins are initially digested with some proteolytic enzyme, like trypsin, into peptides. Then, the peptide mixture is passed through a mass spectrometer, generating MS1 spectra. One prominent peptide at a time is selected from the MS1 spectra and further fragmented into fragment ions, and mass spectrometer will capture the $m/z$ values and intensities of these fragment ions, resulting in a specific mass spectrum signature for each peptide, called the MS2 spectrum. Next, acquired MS2 spectra are matched to a peptide database to detect which peptides are present in the sample. Finally, the peptide profile is used to predict which proteins are more likely to produce the observed peptide set. 

High dynamic range of protein abundance, limitations in digestion and mass spectrometry often lead to ambiguous peptide identification result~\citep{pfeuffer2020epifany}~\citep{serang2010efficient}. In addition, the existence of degenerate peptides and one-hit proteins further complicates the problem~\citep{pfeuffer2020epifany}. Degenerate peptides are those that can be originated from multiple (degenerate) proteins. Those peptides introduce ambiguity in associating detected peptides with their respective proteins. One-hit proteins are those that are backed by single peptide evidence, making it difficult to confidently infer the presence of this protein. The issue is amplified as some peptides are more prone to detection, skewing protein identification towards those producing such peptides. These elements together confound the protein inference process, thereby creating an intricate, complex landscape for protein identification. 

Various approaches have been developed to address the challenges associated with protein inference. ProteinProphet~\citep{nesvizhskii2003statistical}, an early innovator in this field, employs a heuristic-based probabilistic model to estimate protein probabilities, accounting for factors such as shared peptides and the quantity of peptides identified for each protein. PIA~\citep{uszkoreit2015pia}, a rule-based algorithm, conducts maximum parsimony inference, which aims to identify the minimal set of proteins that most accurately accounts for the observed Peptide-Spectrum Matches (PSMs).

In addition to these methods, Bayesian networks have emerged as a highly efficacious technique for protein inference. Fido~\citep{serang2010efficient} was the first to implement Bayesian networks in this domain, incorporating simple yet rational assumptions. Specifically, for proteins sharing degenerate peptides, the method gives preference to those with independent evidence. Concurrently, the ``explain away'' effect reduces the scores for proteins without distinct evidence. {\color{blue}For example, when two proteins share a common peptide and nothing else, they should have the same protein scores because of symmetry. If we give one of the proteins a unique peptide evidence, then the protein score of the one with unique peptide should be elevated, while the one without unique pepitde should be lowered, this is because the protein with unique peptide has already ``explained away'' the common shared peptide, making the protein without unique peptide less likely.}  Epifany~\citep{pfeuffer2020epifany} utilizes a Bayesian network akin to Fido's, but incorporates additional priors to regularize the inference process and employs a rapid approximation inference algorithm to enhance computational efficiency. 
Nevertheless, these techniques are constrained by the inherent limitations of Bayesian networks,
which include high computational costs in terms of time and memory, inability to leverage supplementary features from the peptide search engine, and susceptibility to prior probabilities.

With the advent of neural network advancements, deep learning techniques have delivered promising results in biomedical research, including, but not limited to, prediction of peptide properties from tandem mass spectra~\citep{guan2019prediction}, peak detection~\citep{zohora2019deepiso}, peptide database search~\citep{diann}, and de novo sequencing of peptides~\citep{tran2017novo}~\citep{qiao2021computationally}~\citep{tran2019deep}. However, given that deep learning methods usually require a massive amount of labeled data for training, it is very challenging to apply them in the field of protein inference. The scarcity of labeled data in this field, primarily due to the prohibitive costs of accurately annotating proteins in a biological sample, presents a considerable barrier.

In recent years, a limited number of deep learning-based methods have been proposed to address the protein inference problem. For instance, Barista~\citep{spivak2012direct} trains a binary classification network by treating decoy proteins as negative labels and the remaining proteins as positive. Thereby the classification scores can be directly adopted as the protein scores. However, this methodology can inadvertently infer an inaccurate classification boundary, as not all assumed positive proteins are actually present in a given sample. Secondly, the strategy also runs the risk of overfitting decoy proteins, which are conventionally employed to discern truly present proteins based on a predefined FDR threshold~\citep{elias2007target}. Moreover, the neural network design of Barista \citep{spivak2012direct} does not allow the feature of one protein to affect another, making it unable to take advantage of the ``explain away'' effect of a Bayesian network. 

In contrast, DeepPep~\citep{kim2017deeppep} leverages unsupervised learning to circumvent the problem of label scarcity. Specifically, it utilizes peptide identification scores as labels and trains a model to predict these scores based on all proteins. By sequentially removing each protein from the input, the model can infer the contribution of each protein to each peptide. The final protein score is an aggregation of each protein's contribution to all potential peptides based on their identification scores. Nonetheless, this approach suffers from computational inefficiency, as it necessitates iterating over all proteins for each peptide. Therefore, despite the potential of existing deep learning methods, they remain somewhat marginalized within the protein inference field because of their subpar performance relative to Bayesian networks. {\color{blue}In our experiment, DeepPep~\citep{kim2017deeppep}, a recent deep learning method, generally underperforms with respect to the best-performing Bayesian method by over 25\% ~\citep{pfeuffer2020epifany}. }

In this study, we present GraphPI, a novel deep learning-based framework to address the protein inference problem. Drawing inspiration from Bayesian network techniques, we design a protein-peptide-spectrum graph structure with uniquely crafted node and edge features. This enables us to perceive candidate proteins as interconnected entities rather than isolated individuals. The protein inference problem can be then formulated as a node classification problem with protein scores generated directly from the node classification scores. To process the protein-peptide-spectrum tripartite graph, we employ Graph Neural Networks (GNNs)~\citep{kipf2016semi} as the backbone feature encoder and develop a tailored GNN architecture extending from GraphSAGE~\citep{hamilton2017inductive} to account for the heterogeneity of our graph. To mitigate the label scarcity issue and improve computation efficiency, our model is primarily trained on a set of large and unlabeled public protein datasets from ProteomeXchange\footnote{\url{https://proteomecentral.proteomexchange.org/}} in a semi-supervised learning setting, using pseudo-labels generated by an existing protein inference algorithm as the base model. We further refine these labels by introducing hard negative decoy protein information, allowing the model to exceed the capabilities of the base model and produce improved test results. Finally, we perform self-training to further enhance our model's performance by iteratively refining labels based on their confidence scores. Figure~\ref{fig:overall_structure} presents the overall pipeline of GraphPI. 
Contrary to alternative approaches which necessitate the execution of training or fine-tuning processes for each individual dataset, our analysis indicates that the data pertaining to peptide identification exhibits considerable normalization across all test datasets. This standardization facilitates the application of a single model, which can be trained and subsequently assessed universally, thus circumventing the issue of overfitting. Additionally, this method enhances computational efficiency by mitigating the need for repetitive training processes for disparate datasets.

To the best of our knowledge, we are the first to apply GNNs and a semi-supervised training scheme to the protein inference problem, and the experiments demonstrate that our approach achieves competitive performance across diverse test datasets. Additionally, we leverage the inherently parallelizable structure of neural networks, leading to considerably faster computations in comparison to existing methods. Moreover, our model, pre-trained on a wealth of publicly available datasets, is adept at performing inference instantaneously during real-time applications. As a result, the improvements in efficiency facilitate our model to handle protein inference tasks, seamlessly scaling to accommodate large protein datasets.
\begin{figure}[t!]
\centering
    \includegraphics[width=6.3in]{k_figures/overall_graphPI_structure_revision.eps}  
    %\vspace{-0.55cm}
    \caption{This figure presents the architecture of our protein inference algorithm leveraging GNN for node classification. The process begins with the input of Percolator~\citep{kall2007semi} PSM files into the GNN-based Node Classification module. This module utilizes pseudo-scores from an established protein algorithm to guide the initial classification. Within the module, a tripartite graph is constructed, linking proteins, peptides, and PSMs, as indicated in the detailed view. The algorithm then employs a self-training strategy over multiple iterations to refine the protein scores, as illustrated in the top sequence. Finally, the iterative process yields aggregated confidence scores for each protein, denoted by $y_i$, which are presented on the right. These resulting scores reflect the cumulative learning and adjustment from the iterative self-training, yielding a robust set of protein identifications.}
\label{fig:overall_structure}
\end{figure}



==> chapters/Methodology.tex <==
\section{Methods}


\subsection{Overview}
We present a deep-learning framework, GraphPI, for protein inference that avoids the need for labeled protein datasets, and offers improved computational efficiency compared to existing methods. Our approach leverages a semi-supervised binary classification model that is trained on a set of protein datasets, which are pseudo-labeled by an existing protein inference method. Each dataset is represented as a tripartite graph and encoded using a GNN network that accommodates the heterogeneity of node and edge types.
Following training on the pseudo-labels, we implement a self-training procedure that refines the labels based on protein probability scores followed by a fresh retraining, and we iterate this process for multiple rounds. The final protein scores are calculated as an ensemble of the models from all rounds. To ensure the generalizability of our model to real-world data, we utilize a variety of experimental datasets from published biological research. The following sections delineate our methodology in three parts: 1) Construction of Tri-partite Graph: the conversion of protein datasets into tripartite graphs; 2) GNN Model Architecture: the elaboration of our model's architecture for encoding these graphs into latent representations amenable to deep learning; 3) Training: a detailed exposition of our novel training paradigm. This paradigm leverages the power of semi-supervised learning with an iterative self-training mechanism that begins with pseudo-labels and evolves to deliver refined, reliable inferences.


\subsection{Construction of Tri-partite Graph}
\label{sec:tri-partite graph}
For the protein inference problem, understanding the relationship between proteins, peptides, and their associated PSMs is paramount since the identification of each protein is closely tied to its constituent peptides, which in turn is validated by the confidence of their PSMs. Given the inherent interconnectedness of these components, a graphical formulation naturally emerges as an apt choice. By representing the data as a graph, we can capture the complex dependencies among proteins, peptides, and PSMs through GNNs, and then, we could leverage the learned protein node representation, which consists of multi-hop information from its related peptides and PSMs to generate the protein score. In the following paragraphs, the details of the graph are presented, focusing primarily on the nodes and edges, and their associated features.

\subsubsection{Nodes in the Tri-partite Graph} 
The foundation of our graph lies in its nodes, which are categorized into three specific types: proteins, peptides, and PSMs. We prioritize PSMs over spectra as a node type due to their inherent adaptability in incorporating supplementary features. For instance, peptide search engines such as Percolator~\citep{kall2007semi} rely on a suite of PSM-centric features to compute peptide identification scores. In this study, we primarily utilize the PSM features from Percolator, which are presented as Table S1. In our model, these PSM features are harnessed not just for peptide identification but are further refined to aid in the prediction of protein scores. By doing so, we facilitate an end-to-end training process where peptide identification scores are optimized in alignment with the ultimate goal of predicting protein scores. Moreover, the volume of PSM nodes corresponding to a peptide is deemed valuable; a higher tally of matches between peptides and spectra, especially with elevated identification scores, often indicates a heightened likelihood of peptide presence.

While PSM nodes come with pre-existing features from a database search engine, the nodes representing peptides and proteins lack such attributes. Nonetheless, GNNs necessitate node features. Possible strategies for feature assignment range from designating unique one-hot vectors for each node to allotting universal features (e.g., a vector with all ones) across all nodes. However, a unique one-hot vector for every node tends to restrict the graph learning to be transductive, inhibiting its generalization to datasets with varying node counts and structures. On the other hand, uniform features for peptide and protein nodes might compromise the GNN's ability to differentiate between messages from diverse node types. To circumvent these challenges while maintaining inductive capabilities, we allocate two separate one-hot vectors for protein and peptide nodes. Additionally, learnable embedding layers are applied on top of the one-hot vectors to make them dimensionally equivalent to the PSM node features. This strategy enables our model to distinguish between different types of nodes while retaining the capacity to adapt to diverse datasets.


\subsubsection{Connecting the Dots: Edges in the Tri-partite Graph} 
While nodes represent distinct entities, the true essence of their relationships is captured through edges. Peptides and PSMs are interconnected in a one-to-many relationship, with each PSM associated with a unique peptide-spectra pair. To enable our model to selectively control the flow of information from a specific PSM node to a peptide node, we choose the peptide identification score as the edge weight for each (peptide, PSM) pair, which is defined as $E_{uv}$ for a given source node $u$ and a target node $v$ in the remaining sections. In doing so, a lower identification score signals a weaker presence of a peptide in the sample mixture, thereby indicating that the corresponding PSM node is less reliable for computing the score of its parent protein nodes.

An edge is formed between a protein and a peptide if the peptide appears in the protein. Instead of setting all edge weights to 1, which simply indicates connectivity between peptide and protein nodes, we could incorporate certain prior knowledge into the design. To this end, we integrate a peptide-sharing feature into our graph design by creating a specialized edge attribute $S_{uv}$ between a peptide $u$ and a protein $v$, which is defined as
\begin{align}
    S_{uv} = \left \{
        \begin{aligned}
             & \frac{1}{|C|}, \  \text{if} \ v={\arg max}_k {f(k)} \ \forall k \in C, \text{where} \ C=\{k| A_{uk}=1\} \\
             & 0, \  \text{if} \ v\neq{\arg max}_k {f(k)}
        \end{aligned}
        \right.  
            \label{eq: protein score 1}
\end{align}
Here, $A$ is the bipartite adjacency matrix for peptide and protein, $A_{uv}=1$ indicates a connection between peptide $u$ and protein $v$, and $C$ is the node indexes of the protein nodes that connect to the peptide $u$. $f(\cdot)$, a score indicating if a protein is connected to many high-scoring peptide, is defined as
\begin{align}
    f(k) = \sum_{l \in D}(\mathbbm{1}_{d_i > \epsilon}), \text{where} \ D=\{l | A_{lk} = 1\}
    \label{eq: protein score 2}
\end{align}
where $d_i$ is the maximum peptide identification scores of peptide $i$ (i.e., each score associates with one PSM), and $\epsilon \in [0, 1]$ is a hyper-parameter. 
The peptide-sharing feature discounts a peptide's relevance to its parental proteins if it is connected to multiple proteins. Elaborating, for a peptide that connects to multiple proteins, a surrogate score (i.e., $f(k)$ in Eq.\eqref{eq: protein score 2}) is ascertained for each protein, gauged by the count of top-scoring peptides tethered to it. Subsequent to this, solely the edge weight for the protein with the highest surrogate score is retained, with all others being nullified. The penultimate step involves diminishing the edge weight of this top-scoring protein by a factor of $\frac{1}{|C|}$ as laid out in Eq.\eqref{eq: protein score 1}. The intuition here is that we aim to further mitigate the contribution of a peptide to its parental protein if it is not unique evidence of the protein. In practice, the threshold $\epsilon$ is set at 0.9, a decision stemming from our intention to prioritize peptides with high confidence. Note that in this feature design, although the edge weight between a peptide and a weakly connected protein is set to 0, it is only used as a feature in the subsequent model, and the edge still exists. A schematic depiction of the tri-partite graph is available in Figure~\ref{fig: schema}.

\begin{figure}[t!]
\centering
\begin{subfigure}[t]{1\linewidth}
    \centering
    % \includesvg[height=2.9cm]{figures/swat_graph_deviation.svg}
    \includegraphics[width=5.5in]{k_figures/protein_graph_schema_new.eps}  
    %\vspace{-0.55cm}
    \caption{}
    \label{fig: schema}
\end{subfigure}
%\hspace{\fill} % maximize horizontal separation
\newline
\vspace{0.5cm}
\centering
\begin{subfigure}[t]{1\linewidth}
    \centering
    % \includesvg[height=2.9cm]{figures/wadi_graph_deviation.svg}
\includegraphics[width=5.5in]{k_figures/protein_message_propagation_new.eps}  
       % \vspace{-0.55cm}
    \caption{}
    \label{fig: gnn message passing}
\end{subfigure}
\caption{(a): The schema of the bidirectional tri-partite graph, with $S_{uv}$ and $E_{uv}$ denote as the edge attribute for (protein, peptide) and (peptide, PSM) node pairs respectively, and $x_u$ is an example of the node feature vector for each type of the three nodes (one-hot embedding for protein and peptide nodes, and database search engine features for PSM nodes). (b): An illustrative example of the message passing operation of GNN, where the message update function of each edge type is processed differently.}
\end{figure}


\subsection{GNN Model Architecture} 

Using the tripartite graph as input, we can naturally formulate the protein score generation as a protein node prediction task, utilizing GNNs as the foundational model architecture. Our design draws inspiration from GraphSAGE, a network that elevates message-passing operations through a customized aggregation function. This offers greater flexibility compared to GCNs (Graph Convolutional Neural Networks~\citep{kipf2016semi}), which rely solely on a linear transformation of node features and a subsequent mean aggregation from neighboring nodes. Notably, our model augments GraphSAGE by addressing the inherent heterogeneity of the tripartite graph. This refined architecture is underpinned by two core principles: 1) distinct edge types propagate messages uniquely. 2) different node types update their hidden representations differently.

Formally, given the tri-partite graph $\G=(\E, \V)$, where the set of nodes $\V$ is partitioned into three disjoint subsets: $\V_{\text{pep}}$, $\V_{\text{pro}}$, and $\V_{\text{psm}}$, representing the nodes for peptides, proteins, and PSMs, respectively.
We define the message passing operation between a source node $v \in \V$ and a target node $u \in \V$ as
\begin{align}
a_u^{(k)} &= \sum_{v \in \N_u} m_v^{(k-1)}\\
h_u^{(k)} &= \sigma(W_k \cdot (h_u^{k-1} \mathbin\Vert a_u^{(k)}) + b_k)
\label{eq. message passing}
\end{align}
where $h_u^{k}$ denotes the output feature representation of node $u$ at the $k$-th GNN layer ($h_u^0 = x_u$, the feature of node $u$), $\N_u$ represents the set of neighboring nodes of $u$, $W_k$ and $b_k$ are the learnable weights and biases, and $\sigma$ is a ReLU function. The message $m_v$ propagating from node $v$ to $u$ is uniquely defined for different edge pairs. For node pairs comprising peptides and proteins, i.e., $(u \in \V_{pro}, v \in \V_{pep})$ or vice versa, the message $m_v$ at the $k$-th layer is computed as
\begin{align}
m_v^{(k)} = \sigma(W^{p}_k \cdot (h_v^{(k-1)} \mathbin\Vert E_{uv})+ b^{p}_k)
\label{eq. message function for protein and peptide}
\end{align}
where $E_{uv}$ represents the edge attribute associated with the ($u$, $v$) pair, i.e., the feature that penalizes the peptide having non-unique evidence for the target protein, and $\mathbin\Vert$ denotes a vector concatenation, $W_k^p$ and $b_k^p$ are the weights and biases for the peptide-protein pairs. Conversely, the message between peptides and PSMs, i.e., $(u \in \V_{psm}, v \in \V_{pep})$ or vice versa, is defined as
\begin{align}
m_v^{(k)} = E_{uv} \cdot \sigma(W^{m}_k \cdot h_v^{(k-1)}+ b^{m}_k)
\label{eq. message function for psm and peptide}
\end{align}
where $E_{uv}$ corresponds to the identification score of the source PSM node, $W_k^m$ and $b_k^m$ are the weights and biases for the peptide-PSM pairs. See Figure~\ref{fig: gnn message passing} for a visual illustration of the proposed GNN message passing operation.

It's noteworthy that our model employs a unique set of learnable weights and biases for different edge pair types, capturing the varied distributions across node types. For example, the number of PSM nodes serves as important prior information, as a peptide connected to more PSMs suggests a higher likelihood of occurrence. Similarly, the count of peptides linked to a protein indicates the probability of its target protein's presence. By using specific transformations for these node distributions, our model captures information intrinsic to each node type.

Moreover, we use different message functions for pairs of nodes that have different edge attributes. For the edge attribute between peptides and PSMs, which reflects the probability that a PSM originates from a given peptide, we selectively filter out PSMs that are unlikely to have originated from the peptide directly based on the edge score (shown in Eq.~\eqref{eq. message function for psm and peptide}). On the other hand, for the edge attribute between proteins and peptides, we treat the edge attribute as a feature rather than a filter (shown in Eq.~\eqref{eq. message function for protein and peptide}), as it provides relatively weak prior information. In this way, we let the neural network learn the importance of peptides in relation to a given protein primarily in a data-driven way. 

% \subsection{Model Optimization}
% \subsubsection{Semi-supervised training based on Pseudo-labels}
% We optimize the GNN model architecture through a binary cross-entropy loss on protein nodes, which is defined as
% \begin{align}
%     L = \frac{1}{|\V_{pro}|}\sum_{i\in \V_{pro}} \left[ {\hat{y}_i \log{y_i} + (1-\hat{y}_i) \log {(1-y_i)}} \right]
% \end{align}
% where $\hat{y}_i$ is obtained by passing the GNN output representation $h_i$ of protein $i$ through a learnable one-layer feedforward neural network, i.e., $f_o(\cdot): R^d \rightarrow R$, and $y_i$ corresponds to the true label of protein $i$. That is, the node classification is primarily based on the protein nodes. Since we typically don't have access to the ground truth labels for proteins, we start by using an existing protein algorithm to generate the pseudo-scores for each protein, and then we convert the scores into 1 or 1 based on why it passes the $5\%$ decoy FDR threshold or not. In addition, we intentionally relabel the decoy proteins to negatives, i.e., 0, since this is the information that we already know before the training. 


\subsection{Training}

We train our model under a self-training scheme, which is a classic semi-supervised learning technique that iteratively uses the label generated by the trained model as the training label for the next round of training procedure. This approach hinges on the premise that the efficacy of a new model iteration is closely tied to the quality of the pseudo protein labels from its predecessor.

In a typical self-training setting, a model is initially trained using a small labeled dataset and subsequently applied to a large unlabeled dataset to generate pseudo labels. The same model is then trained on a combination of labeled and pseudo-labeled data, with unlabeled data iteratively added to the training set. However, in our problem setting, we lack labeled data initially, while having access to other protein inference models to generate pseudo labels for the unlabeled data. As a result, we adopt a self-training variation similar to the work~\citep{pang2020self}, in which an existing benchmark model provides the initial labeled dataset.

In this study, our model undergoes training within a binary classification framework. The training loss, binary cross entropy, is mathematically defined as:
\begin{align}
L = \frac{1}{|\V_{pro}|}\sum_{i\in \V_{pro}} \left[ {\hat{y}_i \log{y_i} + (1-\hat{y}_i) \log {(1-y_i)}} \right]
\end{align}
In this formulation, $\hat{y}_i$ represents the predicted label, derived from the GNN output representation $h_i$ of protein $i$ through a trainable one-layer feedforward neural network, denoted as $f_o(\cdot): R^d \rightarrow R$. The term $y_i$ corresponds to the actual label of protein $i$. The classification process predominantly focuses on protein nodes.

Given the typical unavailability of ground truth labels for proteins, our approach employs pseudo labels generated by thresholding the scores from a benchmark model. The threshold is determined based on the False Discovery Rate (FDR); specifically, proteins exceeding a defined FDR threshold (e.g., 0.05 in our experiments) are categorized as positive samples, with the rest deemed negative. Additionally, decoy proteins are explicitly labeled as negative, owing to their inherent absence in biological samples. After the initial training round based on the labels provided by the benchmark model, we replace the previous pseudo labels with the new ones generated by our latest model and retrain our deep learning model accordingly in subsequent self-training rounds.

In each round $i$ (including the initial round, where the training is based on labels provided by the selected benchmark model), the self-learning procedure outputs a learned model $\phi_i$ and returns a list of trained models. Analogous to ensemble learning, we perform an average aggregation of all learned models to obtain the optimal protein score. Specifically, the final protein score for a given protein x is computed as follows:
\begin{align}
score(x) = \frac{1}{t}\sum_{i=1}^{t}\phi_i(x)
\end{align}
where $t$ denotes the total number of self-training rounds.


We employ self-training on several public datasets. Once trained, the model is directly applied to each test dataset to produce the respective protein scores, eliminating the need for re-training. In contrast to methods demanding distinct training or fine-tuning for individual datasets, our findings underscore a pronounced consistency in peptide identification data across all examined datasets. Such uniformity allows us to deploy a single, universally adaptable model, mitigating the problem of overfitting. Moreover, this approach increases computational efficiency by reducing the need for redundant training procedures for different datasets.


\subsection{Implementation}

\subsubsection{Experimental Setting}
In our experiments, we select Epifany as the base model to generate the initial pseudo labels due to its relative computational efficiency compared to other models and competing performance, as demonstrated in their original paper.

We adopted the Adam optimizer with a learning rate of 0.001. We use torch\_geometric with version 2.1.0 for the implementation of GNN.
The model is composed of six GNN layers, with node and edge hidden dimensions set to 100. In addition, our model is trained on a single Nvidia RTX4090 graphics card over 1000 epochs, and the parameters leading to the best validation loss are stored. 

The software versions and configurations in our experiments are all listed in Table S3 .


\subsubsection{Trainging Datasets} 
\label{sec: training datasets}
The training datasets are public protein datasets downloaded from ProteomeXchange. To avoid over-fitting to a specific benchmark dataset used in our experiment, those datasets are selected randomly, and processed with Comet~\citep{eng2015deeper} search and Percolator~\citep{kall2007semi} for peptide database search, with respect to their experimental specifications.


The following are the final datasets used for training: PXD004789~\citep{kreutz2017response}, PXD005388~\citep{meier2017organoruthenium}, PXD006640~\citep{venkatraman2017proteomic}, PXD010319~\citep{meier2017organoruthenium}, PXD022881~\citep{bhat2021combined}, PXD023593~\citep{lupton2021cryo}, PXD025701~\citep{mumtaz2022secreted}, PXD026991~\citep{fischer2022supt3h}, PXD030448~\citep{hotta2022eml2}, PXD032035~\citep{liu2022sars}, PXD032284~\citep{lo2023development}, PXD036171~\citep{su2023study}, PXD039272~\citep{hsu2020trop2}, PXD034012~\citep{cela2022proteomic}, PXD023034~\citep{Zawily2023}, PXD030330~\citep{Jaffray2023}, and PXD035125~\citep{Herman2022}, the links and search parameters of which are listed in Table 1 and 2 of the Supplementary Material.


\subsubsection{Test Datasets}
We evaluated our algorithm on the four MS/MS datasets: iPRG2016~\citep{iprg2016}, UPS2~\citep{ups2}, 18Mix~\citep{18mix}, and Yeast~\citep{ramakrishnan2009gold}. These datasets provides us with ground truth labels for evaluating entrapment FDR. Among these datasets, iPRG2016 was specifically curated to test protein inference algorithms on proteins that share peptides. 18Mix and Yeast also contain peptide-sharing proteins. A detailed description of these datasets are provided in the Supplementary Material.

To process the tandem MS data, we first converted and centroided the raw files with msConvert. For UPS2, we do not need to generate decoy proteins since they are already provided by the fasta file. For other datasets, the provided fasta file was used to generate a decoy database through shuffling of amino acid with the OpenMS DecoyDatabase tool. Then, spectra were searched using Comet allowing 10 ppm precursor mass tolerance, 0.01 Da fragment mass tolerance, and one missed cleavage for fully tryptic peptides (for 18Mix, the precursor and fragment mass tolerance is set to 1.005 Da since it comes from a low resolution instrument). Carbamidomethylation(C) is selected as the fixed modification except Yeast (which does not undergo alkylation), and oxidation(M) the variable one. Then, we extracted additional features from the Comet search, and feed them into Percolator to obtain better peptide scores.


\subsubsection{Benchmark Methods}
We used the following four popular and representative methods to compare against our model: Epifany \citep{pfeuffer2020epifany}, Fido \citep{serang2010efficient}, PIA \citep{uszkoreit2015pia}, and DeepPep \citep{kim2017deeppep}. They are either based on parsimony, probability, Bayesian, or
deep learning approaches, covering the majority of the approaches to this problem. 

Leveraging PSM features from Percolator, each method derives a probability score for individual proteins. The probability output of each model is used to rank the proteins. Groups of identically connected proteins are treated as one single protein group during inference. When we are referring to the number of proteins, such groups contribute only one per group, instead of contributing once per protein.


==> chapters/toc.tex <==
\section{For TOC Only}

\begin{figure}
    \centering
    \includegraphics[width=3in]{k_figures/TOC.eps}    %\caption{Caption}
    %\label{fig:enter-label}
\end{figure}
